HuMMan: Multi-Modal 4D Human Dataset for Versatile Sensing and Modeling

4D human sensing and modeling are fundamental tasks in vision and graphics with numerous applications. With the advances of new sensors and algorithms, there is an increasing demand for more versatile datasets. In this work, we contribute HuMMan, a large-scale multi-modal 4D human dataset with 1000 human subjects, 400k sequences and 60M frames. HuMMan has several appealing properties: 1) multi-modal data and annotations including color images, point clouds, keypoints, SMPL parameters, and textured meshes; 2) popular mobile device is included in the sensor suite; 3) a set of 500 actions, designed to cover fundamental movements; 4) multiple tasks such as action recognition, pose estimation, parametric human recovery, and textured mesh reconstruction are supported and evaluated. Extensive experiments on HuMMan voice the need for further study on challenges such as fine-grained action recognition, dynamic human mesh reconstruction, point cloud-based parametric human recovery, and cross-device domain gaps.

==> sections/99_archive.tex <==
\section{Hardware}

\begin{figure}
  \includegraphics[width=\linewidth]{img/hardware_img/stack2.pdf}
  \caption{Second stack of the framework mounting 8 cameras on each side and an iPhone}
  \label{fig:stack2}
\end{figure}

\begin{figure}
  \includegraphics[width=\linewidth]{img/hardware_img/stack3.pdf}
  \caption{Third stack of the framework mounting 2 cameras in symmetry to cover views at high altitude above human}
  \label{fig:stack3}
\end{figure}

\begin{figure}
  \includegraphics[width=\linewidth]{img/hardware_img/device.pdf}
  \caption{Azure Kinect DK\cite{Kinect1}}
  \label{fig:kinect}
\end{figure}

\begin{figure}
 \includegraphics[width=0.5\linewidth]{img/hardware_img/camera.pdf}
 \caption{Azure Kinect DK and iPhone and their installation}
 \label{fig:camera}
\end{figure}

\begin{figure}
  \includegraphics[width=0.2\linewidth]{img/hardware_img/phone.pdf}
  \caption{A screen shot of RGB-D data recording application we developed on iPhone}
  \label{fig:iphone}
\end{figure}

\begin{figure}
  \includegraphics[width=0.2\linewidth]{img/hardware_img/evatitlephoto.pdf}
  \caption{Artec Eva handheld 3D scanner}
  \label{fig:eva}
\end{figure}

\subsection{Consumer-level RGB-D Sensor}

Azure Kinect DK as the most popular RGB-D camera for research and industrial uses, can be considered as an integration of USB devices including a RGB camera, a depth camera, infrared emitters and 7 microphone array. We select the operating mode for color camera with $1920\times1080$ ($H\times V$) resolution, 30 FPS and $90^{\circ} \times59^{\circ}$ FOV. We select the "NFOV unbinned" operating mode for depth camera with $640\times576$ ($H\times V$), 30 FPS and $90^{\circ} \times59^{\circ}$ FOV, which has the most overlaps of view with RGB camera and the densest point clouds. The operating range of this mode is between 0.5m to 3.86m. Point clouds from depth images are less accurate by far distance. The random error standard deviation of each pixel depth is not larger than 17mm and the typical systematic error of the depth sensor is less than 11 mm + 0.1\% of distance. Because of the limited FOV and capture distance of the sensors, we design an aluminium framework to arrange our cameras(Figure \ref{fig:framework}). It has four stacks of equilateral octagon with 1.7m length of the sides and 2.05m length from a side to its center. From the base to the top, 8 Kinect cameras are arranged on 8 sides of the second stack with ranged height and 2 Kinect cameras are arranged on the third stack in symmetry (Figure \ref{fig:stack2} and Figure \ref{fig:stack3}). In this case, when people stand or jump or lay down in the center, their whole body can be covered in at least 2 camera's view range. Each camera is screwed on a ball head for tripod while each ball head is fixed on an aluminium slider inserted into the framework's v-slots. Therefore, camera positions can be easily adjusted and fixed to avoid camera movement during the data collection. Azure Kinect DK allows multiple devices to be synchronized by external sync trigger signals through audio cables. We use the Daisy-Chain synchronization configuration in which devices are connected in serial and triggered from a master device. Depth information of one devices is collected from its infrared sensor and 9 infrared pulses received by the sensor to derive one depth frame. To prevent the lasers from interfering with one another, multiple devices must have their lighting sequence of infrared laser. Because of differences between the camera clock and the device firmware clock, a minimum pulse width needs $160\mu s$. The idle time between two pulses is $1450\mu s$. This allows 9 additional devices to emit their individual pulses between one idle time period, so the maximum number of synchronized devices is 10.

\subsection{Mobile RGB-D Sensor}
The most advanced mobile devices, like iPhone 12 Pro, iPhone 13 Pro and iPad Pro are equipped with a Light Detection And Ranging sensor(Lidar), which provides depth information. The ARKit SDK allows us to access the device's RGB-D information in 60 frames per second. Each frame contains a RGB image of $1920 \times 1440$ ($H\times V$) and a depth image of $256 \times 192$ ($H\times V$). This also comes with a corresponding confidence map, in which the confidence of each depth pixel has 3 values from 0 to 2, depending on the detecting surface properties. Kinect camera, iPhone camera and computer all have their individual device time.Because there is no hardware-based approach to synchronize iPhone camera and Kinect camera, we decide to solve it by a network communication approach. At the beginning of recording RGB-D videos, a request of iPhone system clock time is sent by computer to iPhone to calculate their system time difference. The $travel \ time$ between two system is $t_{travel}$. $Local\ system\ time$ when computer sends the request is $t_{pc}$ and $iPhone\ system\ time$ when iPhone receives it is $t_{iPhone}$. The time difference of their clock time is $\triangle t_{iPhone2pc} = t_{pc} - t_{iPhone} + \frac{t_{round}}{2}$. After the first frame is recorded, there are three time data saved: $Kinect\ first\ frame\ time $, $t_{Kinect0}$; $local\ first\ frame \ system\ time$, $t_{pc0}$ and $iPhone\ first\ frame\ time$, $t_{iPhone0}$. The time difference between Kinect system and computer system is $\triangle t_{pc2Kinect} = t_{Kinect0} - t_{pc0}$. The time difference between iPhone system and Kinect system can be derived as $\triangle t_{iPhone2Kinect} = \triangle t_{iPhone2pc} + \triangle t_{pc2Kinect}$. The iPhone system time, corresponding to Kinect system time, should be $t_{iPhone} = t_{Kinect}-\triangle t_{iPhone2Kinect}$. Because iPhone's RGB-D frame contains an independent time, its inner time difference between iPhone system and iPhone frame is $\triangle t_{iPhone2ARKit} = t_{ARKit0} - t_{iPhone0}$. Therefor iPhone frame time, corresponding to Kinect system time, should be $t_{ARKit} = t_{iPhone} + \triangle t_{iPhone2ARKit} - t_{offset}$. Two frames from iPhone and Kinect with $|t_{ARKit} - t_{Kinect}| < 16.7ms$ are considered as synchronized frames.

\subsection{High Resolution Scanner}
Artec Eva(Figure\ref{fig:eva}), a product of Artec 3D, is a fast handheld 3D scanner for professionals.  Using structured light, it has 3D point accuracy up to 0.1 mm and 3D resolution, up to 0.2 mm. 3D accuracy can be varied over distance, up to	0.1-0.3 mm/m. We use it for generating accurate point cloud and high-resolution textured human mesh.

\subsection{Calibration}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/before_and_after_icp.png}
    \caption{Reconstruction results. Left: Before ICP. Right: After ICP}
    \label{fig:my_label}
\end{figure}

\section{Toolchain}
their corresponding human bounding box. In practice, as only one person is expected to appear in our setting, we select the largest bounding box if there are multiple detection results



\section{Experiments}

% @zengailing
% 500 actions analysis
% Table
\begin{table}[h]%
\caption{The cross-dataset validation of 2D Keypoint Detection on \name. The test dataset is \name by default. * means the model is finetuned on \name. The input size is 385$\times$288. \emph{Data} in this table means the training data.}
%  Training and testing on \name. 
%HPE methods on the test-dev set of the COCO dataset using AP measure (AP.5 means AP at OKS = 0.50, AP.75 means AP at OKS = 0.75, AP(M) is used for medium objects, AP(L) is used for large objects). The best two scores are marked in red and blue, respectively.
\label{tab:cross_data_2dpose}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{c|llllll}
  \toprule
  Method  & Data& AP&AP.5&AP.75&AR \\
  \midrule
  \multirow{3}{*}{Simple-Res50}  & COCO& &&&\\
   & \name&  &&&&\\
   & \name *&  &&&&\\
  \midrule
  \multirow{3}{*}{Simple-Res152}  & COCO&&&&\\
   & \name&   &&&&\\
   & \name *&   &&&&\\
  \midrule
  \multirow{3}{*}{LiteHRNet-w30} & COCO&&&&\\
  &  \name& & &&&\\
  &  \name*& & &&&\\
  \midrule
  \multirow{3}{*}{HRNet-w32-dark} & COCO&&&&\\
   & \name&  &&&&\\
  & \name *&  &&&&\\
  \midrule
  \multirow{3}{*}{HRNet-w48-dark} & COCO&&&&\\
   & \name& &&&&\\
   & \name *& &&&&\\
%   \midrule
%   \multirow{3}{*}{HRNet-w48} &Halpe&  &&&&\\
%   &\name&  &&&&\\
%   &\name *&  &&&&\\
%   \midrule
%   \multirow{3}{*}{HRNet-w48} & Posetrack18& &&&&\\
%   & \name& &&&&\\
%   & \name *& &&&&\\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

% Table
\begin{table}[h]%
\caption{Cross device validation of 2D Keypoint Detection on \name. The method is HRNet-w48-dark by default.}
\label{tab:cross_device_2dpose}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{cc|llll}
  \toprule
  Kinect & iPhone & AP&AP.5&AP.75&AR  \\
  \midrule
  \checkmark & - & & & & \\
   - & \checkmark & &  & & \\
   \checkmark & \checkmark & &  & & \\

  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%


% Table
\begin{table}[h]%
\caption{Cross dataset validation of 2D Keypoint Detection. The training set is \name. The method is HRNet-w48-dark. \TODO{single person set? finetune model}}
\label{tab:comp_data_2dpose}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{c|llll}
  \toprule
  Test sets & AP&AP.5&AP.75&AR  \\
  \midrule
    COCO &&&& \\
    MPII &&&& \\ 
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

\subsection{3D Keypoint Detection}
\input{tables/7_3d_keypoint_crossdata}
\TODO{@Zeng Ailing}


\subsection{Multi-Modal Annotations}
\TODO{@Zeng Ailing}

\input{tables/7_supervision_signals}
\input{tables/7_3d_multitask_action_pose}
We study the usefulness of our multi-modal annotations in two settings. 
%
First, it is a common practice to mix datasets with keypoints annotations and that with SMPL annotations in training for 3D parametric model recovery. As \name provides both keypoints and SMPL annotations, we experiment several types of supervision signals in \Tab\ref{tab:supervision_signals}, that shows having multiple annotations improve model performance.
%
Second, inspired by recent works \cite{} that explore multi-task joint training, we implement two baselines in \Tab\ref{tab:3d_multitask_action_pose} to simultaneous utilize action labels and keypoint annotations. The shows indicate that action recognition and pose estimation have certain inherent connection and are complementary to each other.

==> tables/7_3d_keypoint_crossdata.tex <==

% Table
\begin{table}[h]% 
\caption{Benchmark of Cross-Dataset validation on 3D Keypoint Detection.}
\label{tab:cross_device_3dpose}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{lcccc}
  \toprule
  Method&Train&Test& MPJPE$\downarrow$  & PA-MPJPE$\downarrow$  \\\hline
    \multirow{6}{*}{FCN~\cite{martinez2017simple}}	&\multirow{2}{*}{H36M}	&Kinect&	125.5&	76.5\\
    & &	iPhone	&120.7	&73.1\\
    \cmidrule{2-5}
    &	\multirow{2}{*}{Kinect}&	H36M&	65.8&	41.5\\
    &	&MPI	&& \\	
    \cmidrule{2-5}
    & H36M&	\multirow{2}{*}{AIST++}&	133.9	&73.1\\
    & Kinect	&&	116.4	&67.2\\\hline
    \multirow{6}{*}{Video3d~\cite{pavllo20193d}}&\multirow{2}{*}{H36M}	&Kinect&118.5&	73.4\\
    &	& 	iPhone	&113.8&	70.9\\
    \cmidrule{2-5}
    &\multirow{2}{*}{Kinect}&H36M&63.1&	40.2\\
    &	&	MPI	& &\\	
    \cmidrule{2-5}
    &	H36M&	\multirow{2}{*}{AIST++}&	128.5&	72.0\\
    &	 Kinect	&&	109.2	&63.5\\

  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%



==> tables/7_3d_multitask_action_pose.tex <==
% Table
\begin{table}[h]%
\caption{Benchmark of Multi-task on 3D Keypoint Detection and Action Recognition.}
\label{tab:3d_multitask_action_pose}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{lcc}
  \toprule
  Method  & MPJPE$\downarrow$  &PA-MPJPE$\downarrow$ \\
  \midrule
  Video3d (T=27)~\cite{pavllo20193d} & 73.1&43.5\\
  Video3d (T=27)~\cite{pavllo20193d} w/Action  & 75.3&44.1\\
  \bottomrule
    Method  & Top-1 (\%)$\uparrow$ &Top-5 (\%)$\uparrow$ \\
  \midrule
  ST-GCN~\cite{yan2018spatial} & 72.5	&94.3\\
  ST-GCN~\cite{yan2018spatial} w/Pose& 72.1	&94.2\\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

==> tables/7_3d_pose_estimation.tex <==
% Table
\begin{table}%
\caption{Pose and Shape Estimation (\name). Training and testing on \name.}
\label{tab:pose_and_shape_estimation}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{lll}
  \toprule
  Method & MPJPE & PA-MPJPE \\
  \midrule
  HMR  &  & \\
  SPIN &  & \\
  VIBE &  & \\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

% Table
\begin{table}%
\caption{Pose and Shape Estimation (cross device).}
\label{tab:pose_and_shape_estimation}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{ccll}
  \toprule
  Kinect & iPhone & MPJPE & PA-MPJPE \\
  \midrule
  \checkmark & - & & \\
  - & \checkmark & & \\
  \checkmark & \checkmark & & \\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

% Table
\begin{table}%
\caption{Pose and Shape Estimation (cross dataset). Testing on a standard benchmark.}
\label{tab:pose_and_shape_estimation}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{ccll}
  \toprule
  Standard & \name & MPJPE & PA-MPJPE \\
  \midrule
  \checkmark & - &  &  \\
  - & \checkmark &  &  \\
  \checkmark & \checkmark &  &  \\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%

==> tables/7_cross_action.tex <==

\begin{table}[htbp]
\caption{Cross dataset setting: pretrained on \name, test state-of-the-art methods on existing datasets~\cite{} in terms of Top-1 and Top-5 accuracy(\%). }
\begin{center}
\vspace{-0.3cm}
\small
{
\begin{tabular}{c|cc|cc}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{\textbf{Top-1 (\%)}}& \multicolumn{2}{c}{\textbf{Top-5 (\%) }}\\  
& X-Sub  & X-View  &   X-Sub  &  X-Set  \\
\toprule
% ST-GCN~\cite{yan2018spatial} & 52.1& 48.5&86.2 &84.9\\
% 2s-AGCN~\cite{shi2019skeleton}& 54.5& 49.7& 87.8&86.1\\
% HCSF-GNN~\cite{zeng2021learning} & 55.7&50.3& 88.2& 87.5\\
% PoseC3D~\cite{duan2021revisiting} &\textbf{55.8} &\textbf{50.5}&\textbf{88.6} &\textbf{87.9} \\
\bottomrule
\end{tabular}}
\end{center}
\label{tab:ntu}
\end{table}
% todo: 1. cross-dataset finetune (fc+softmax); 2. wholebody v.s. main poses as input


==> tables/7_supervision_signals.tex <==
\begin{table}[t]
{
\setlength{\tabcolsep}{4pt}
\caption{Supervision Signals.}
\label{tab:supervision_signals}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{cccc}
  \toprule
  Keypoints & SMPL & MPJPE $\downarrow$ & PA-MPJPE $\downarrow$ \\
  \midrule
  \checkmark & - & 58.16 & 39.78 \\
  - & \checkmark & 61.69 & 40.36 \\
  \checkmark & \checkmark &  54.78 & 36.14\\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
}
\end{table}

	



==> tables/7_transferability.tex <==
% Table
\begin{table}
{
\setlength{\tabcolsep}{4pt}
\caption{Transferability to in-the-wild 3D human recovery. Evaluated on 3DPW test set.}
\label{tab:transferability}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{ccccc}
  \toprule
  Standard & \name & Synthetic BG & MPJPE & PA-MPJPE \\
  \midrule
  \checkmark & - & - &  &  \\
  - & \checkmark & - &  &  \\
  \checkmark & \checkmark & - &  &  \\
  - & \checkmark & \checkmark &  &  \\
  \checkmark & \checkmark & \checkmark &  \\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
}
\end{table}



% % Table
% \begin{table}%
% \caption{Joint training. Keypoint Detection + Action Recognition.}
% \label{tab:pose_and_shape_estimation}
% \begin{minipage}{\columnwidth}
% \begin{center}
% \begin{tabular}{ccll}
%   \toprule
%   Action & 2DJoint & 3DJoint&  \\
%   \midrule
%   \checkmark & - &  &  \\
%   - & \checkmark &  &  \\
%   \checkmark & \checkmark &  &  \\
%   \bottomrule
% \end{tabular}
% \end{center}
% \bigskip\centering
% \end{minipage}
% \end{table}%

% % Table
% \begin{table}%
% \caption{Joint training. Ablation on supervision signal for Pose and Shape estimation.}
% \label{tab:pose_and_shape_estimation}
% \begin{minipage}{\columnwidth}
% \begin{center}
% \begin{tabular}{ccll}
%   \toprule
%   Keypoints & SMPL & MPJPE & PA-MPJPE \\
%   \midrule
%   \checkmark & - &  &  \\
%   - & \checkmark &  &  \\
%   \checkmark & \checkmark &  &  \\
%   \bottomrule
% \end{tabular}
% \end{center}
% \bigskip\centering
% \end{minipage}
% \end{table}%

==> tables/9_2d_keypoint_crossdata.tex <==
\begin{table}[h]%
\caption{Benchmark of 2D Keypoint Detection. Input image size is 384*288.}
% todo: finetune on coco 
\label{tab:2d_keypoint}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{lcccc}
  \toprule
  Method  & Train & Test &$AP^{50}\uparrow$  &$AP^{75}\uparrow$\\
  \midrule
    CPN~\cite{chen2018cascaded}&\multirow{3}{*}{COCO}&\multirow{3}{*}{Kinect}&0.57&0.78\\
    HRNet~\cite{sun2019hrnet}&&&	0.61&	0.80\\
    Lite-HRNet~\cite{yu2021lite}&&&	0.55&	0.73\\
    \midrule
    CPN~\cite{chen2018cascaded}	&\multirow{3}{*}{COCO}&	\multirow{3}{*}{iPhone}	&0.62	&0.81\\
    HRNet~\cite{sun2019hrnet}&&	&	0.66	&0.84\\
    Lite-HRNet~\cite{yu2021lite}&&		&0.60	&0.79\\
    \midrule
    CPN~\cite{chen2018cascaded}	&\multirow{3}{*}{Kinect}&\multirow{3}{*}{Kinect}&	0.86&	0.93\\
    HRNet~\cite{sun2019hrnet}&&&0.91&0.97\\
    Lite-HRNet~\cite{yu2021lite}&&&	0.87&	0.93\\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\end{minipage}
\end{table}%
